MatchU: Matching Unseen Objects for 6D Pose Estimation from RGB-D Images

Recent learning methods for object pose estimation require resource-intensive training for each individual object instance or category, hampering their scalability in real applications when confronted with previously unseen objects. In this paper, we propose MatchU, a Fuse-Describe-Match strategy for 6D pose estimation from RGB-D images. MatchU is a generic approach that fuses 2D texture and 3D geometric cues for 6D pose prediction of unseen objects. We rely on learning geometric 3D descriptors that are rotation-invariant by design. By encoding pose-agnostic geometry, the learned descriptors naturally generalize to unseen objects and capture symmetries. To tackle ambiguous associations using 3D geometry only, we fuse additional RGB information into our descriptor. This is achieved through a novel attention-based mechanism that fuses cross-modal information, together with a matching loss that leverages the latent space learned from RGB data to guide the descriptor learning process. Extensive experiments reveal the generalizability of both the RGB-D fusion strategy as well as the descriptor efficacy. Benefiting from the novel designs, MatchU surpasses all existing methods by a significant margin in terms of both accuracy and speed, even without the requirement of expensive re-training or rendering.

==> sec/media/tables.tex <==
\section{Experiments and Results}
\label{sec:experiments_and_results}

\subsection{Datasets and evaluation metrics}
\paragraph{Datasets.} Inspired by ZeroPose \cite{zeropose} and MegaPose \cite{megapose}, we utilize the PBR rendered Google-Scanned-Objects (GSO) dataset \cite{gso} provided by Megapose for training our model. Following the official split of GSO, we use 846 objects for training and the remaining objects for validation. To evaluate our method on the task of unseen object pose estimation, we employ five core BOP datasets as our testing set: LINEMOD-Occusion, T-LESS\cite{hodan2017tless}, TUDL, ICBIN, and YCB-V\cite{xiang2018posecnn}, where their CAD models and images are not available during the training.

\paragraph{Metrics.} Following the BOP challenge, we calculate the error of an estimated pose with respect to the ground-truth pose using three pose-error functions: Visible Surface Discrepancy (VSD), Maximum Symmetry-aware Surface Distance (MSSD), and Maximum Symmetry-aware Projection Distance (MSPD). VSD considers only the visible parts of the object and treats indistinguishable poses as equivalent. MSSD takes into account pre-identified global object symmetries and measures the surface deviation in 3D, while MSPD considers object symmetries and measures the perceivable deviation. The recall of each error is calculated using various thresholds. The average recall of each item, denoted as $AR = (AR_{VSD} + AR_{MSSD} + AR_{MSPD})/3$, serves as the overall benchmark metric.


\subsection{Training and Implementation}
\paragraph{Point cloud feature extraction.} We take RoITr\cite{roitr} network as our backbone to extract rotation-invariant point descriptors. For each observed depth image, we sample at most 2048 points as the target point cloud and the same number is applied for sampling points from the CAD model surface as the source point cloud. We take a 3-layer encoder with the stride of 4,2,2 respectively to down-sample the point cloud into 128 superpoints. An Adam optimizer with an initial learning rate of 1e-4, which is exponentially decayed by 0.05 after each epoch. In all the experiments, we selected 128 superpoint correspondences with the highest scores. Based on each superpoint correspondence, mutual top-3 point correspondences whose confidence scores are larger than 0.05 are further extracted as the point correspondences.

\paragraph{Virtual feature extraction.} We follow the implementation of LoFTR\cite{sun2021loftr} by using a modified ResNet18 as the local 2D feature backbone, extracting superpixel with $1/64$ resolution of the original input image crop. 


\subsection{Evaluation on BOP Core Benchmark Datasets}
\junwen{Table\ref{tbl:main table}: main results compare to baselines}
% \begin{table*}[t]
%     \begin{tabular}{lccccccccc}
%     \hline
%         \textbf{Method} & \textbf{Multi-Hypo.} & \textbf{Refinement} & \textbf{LMO} & \textbf{TLESS} & \textbf{TUDL} & \textbf{IC-BIN} & \textbf{YCBV} & \textbf{Mean} & \textbf{Time(s)} \\ \hline
%         OSOP & \ding{55} & - & 39.3 & - & - & - & \textbf{52.9} & - & 0.47 \\ 
%         Megapose & \ding{51} & - & 18.7 & 19.7 & 20.5 & 15.3 & 13.9 & 17.6 & 2.5 \\ 
%         ZeroPose & \ding{55} & - & 26.1 & 24.3 & 61.1 & 24.7 & 29.5 & 33.9 & 0.30 \\ 
%         Ours & \ding{55} & - & \textbf{53.2} & \textbf{33.5} & \textbf{70.0} & \textbf{26.3} & 50.5 & \textbf{46.7} & 0.13 \\ \hline

%         % \hline
%         % Ours (kun) & \ding{55} & Megapose-RGB & \textbf{55.6} & - & - & - & - & - & - \\ \hline

        
%         Drost, PPF & \ding{51} & ICP & 52.7 & - & - & - & 34.4 & - & 15.95 \\ 
%         OSOP & \ding{51} & ICP & 48.2 & - & - & - & 57.2 & 52.7 & 5.44 \\ 
%         Ours & \ding{51} & ICP & \textbf{59.2} & \textbf{50.2} & \textbf{81.1} & \textbf{44.7} & \textbf{58.6} & \textbf{58.3} & 0.7 \\ \hline
%         Megapose & \ding{51} & Megapose-RGBD & 58.3 & 54.3 & 71.2 & 37.1 & 63.3 & 56.9 & 35.4 \\ 
%         ZeroPose & \ding{51} & Megapose-RGBD & 56.2 & 53.3 & \textbf{87.2} & 41.8 & 58.4 & 59.4 & 9.7 \\ 
%         Ours & \ding{51} & Megapose-RGB & \textbf{61.1} & \textbf{55.7} & 85.4 & \textbf{47.2} & \textbf{64.5} & \textbf{62.8} & 2.1 \\ \hline
%     \end{tabular}
%     \captionsetup{width=\textwidth} % Center the caption
%     \caption{Quantitative results of Average Recall(AR) on BOP5 core benchmark datasets for unseen object pose estimation task. Our method exhibits superior performance by large margins compared to other baselines without any refinement. The results are boosted after applying multi-hypothesis and ICP refinements or Megapose-RGB refiner.}
%     \end{table*}




\begin{table*}[t]
\begin{tabular}
% {lcccccccccccc}
{@{\hspace{5pt}}l@{\hspace{5pt}}l@{\hspace{10pt}}c@{\hspace{10pt}}c@{\hspace{10pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{Method}& \multirow{2}{*}{MH} & \multicolumn{2}{l}{Instance Localization}  & \multirow{2}{*}{Refine.} & \multirow{2}{*}{LMO} & \multirow{2}{*}{TLESS} & \multirow{2}{*}{TUDL} & \multirow{2}{*}{ICBIN} & \multirow{2}{*}{YCBV} & \multirow{2}{*}{Mean} & \multirow{2}{*}{Time(s)} \\
\multicolumn{2}{c}{}&  &zero-shot &trained &  &  & & & & & \\ \hline
\multirow{5}{*}{\begin{tabular}[l]{@{}l@{}}one hypo.\\no refinement \end{tabular}} & ZeroPose  &  & \ding{51} &  &  & 26.0  & 17.8 &  41.2 & 17.7  & 25.7  & 33.1  & 0.30  \\
% Ours   & \ding{51}    & \ding{51}  & &    &     &   &  \textbf{56.2}   & \textbf{49.0}  &   &  &     &      &    \\ 
&OSOP  &   & \ding{51} &  &  & 39.3  & -  &-  & -  &\textbf{52.9}  &  & 0.47      \\
&ZeroPose &    &  & \ding{51}  &  & 26.1  & 24.3  & 61.1 & 24.7 & 29.5 & 33.1 & 0.30 \\
&MegaPose &    &  & \ding{51}  &  & 18.7  & 19.7  & 20.5 & 15.3 & 13.9 & 17.6 & 2.5  \\
&Ours(Fast)  &  & \ding{51} & & & \textbf{52.6} & \textbf{42.9}  & \textbf{70.0} & \textbf{36.7} & 50.5 & \textbf{46.7} & 0.13 \\
\hline
\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}multi-hypo.\\no refinement \end{tabular}} &OSOP  & \ding{51}  & \ding{51} &  &  & 46.2  & - &- & - & 54.2 &-  & 0.47 \\
& Ours(Accurate) & \ding{51} & \ding{51} &  & &  \textbf{56.2} & \textbf{50.6} & \textbf{75.6} &\textbf{42.2} &\textbf{60.8} &  \textbf{55.4}  & 1.03 \\ 
\hline
\multirow{5}{*}{\begin{tabular}[l]{@{}l@{}} zero-shot,\\refinement\\ \end{tabular}} & DrostPPF  &\ding{51}   & \ding{51} &  & \ding{51} &52.7 & - & - & - & 34.4 & - & 15.95  \\
&PPF + Zephyr &\ding{51}  & \ding{51}  &  & \ding{51} & 59.8 & - & -  & -  & 51.6 & -  & 15.95 \\
&OSOP   & \ding{51}  & \ding{51}  &  & \ding{51}  & 48.2 & - & - & - & 57.2 & -  & 5.44 \\
&ZeroPose  & \ding{51} & \ding{51} & & \ding{51}  & 49.1 & 34.0 & 74.5 & 39.0 & 57.7 & 59.4 & 9.76 \\
&Megapose  & \ding{51} & \ding{51} & & \ding{51}  & 62.6 & 48.7 & 85.1 & 46.7 & 76.4 & 59.4 & 9.76 \\
&Ours(Accurate) & \ding{51} & \ding{51} & &\ding{51} &\textbf{64.4} & \textbf{54.7} & \textbf{89.8} & \textbf{44.2} & \textbf{72.6} & \textbf{64.7} &1.99\\
\hline

\multirow{3}{*}{\begin{tabular}[l]{@{}l@{}} trained detector,\\no refinement\\ \end{tabular}} &OVE6D  & \ding{51} &    &  \ding{51} &  & 62.7  & 52.3  & - & - & - & - & - \\
&GCPose & \ding{51}  &  & \ding{51} &  & 65.2  & 67.9  &92.6  &-  &-  & -  &  -  \\
&Ours(Accurate) & \ding{51} & & \ding{51} & &\textbf{66.8} & 65.1 & \textbf{93.1} & \textbf{43.9} & \textbf{65.8} & \textbf{66.9} &5.6\\
\hline
\multirow{5}{*}{\begin{tabular}[l]{@{}l@{}} trained detector,\\ refinement\\ \end{tabular}}& OVE6D  & \ding{51}      & &\ding{51} & \ding{51}  & 62.7  & 54.6   & -     & -   & -  & -   & - \\
&HybridPPF  & \ding{51}  & &\ding{51} & \ding{51}  & 63.1  & 65.5   & 92.0  & -   & -  & -  & -  \\
&Megapose   & \ding{51}  & &\ding{51} & \ding{51}  & 58.3  & 54.3   & 71.2  & 37.1 & 63.3  & 56.8   & 35.5  \\
&ZeroPose   & \ding{51}  & &\ding{51} & \ding{51}  & 56.2  & 53.3   & 87.2  & 41.8 & 58.4 & 59.4  & 9.76                    \\
&Ours(Accurate) & \ding{51} & & \ding{51} & \ding{51} &\textbf{68.0} & \textbf{66.8} & \textbf{95.7} & \textbf{47.4} & \textbf{75.6} & \textbf{70.7}  &5.6\\ 
% Ours                    & \ding{51}   & \ding{51}              &                    & \ding{51}                           & \textcolor{gray}{\textbf{61.1}}        & \textcolor{gray}{\textbf{55.7}}        & \textcolor{gray}{\textbf{85.4}}        & \textcolor{gray}{\textbf{47.2}}        & \textcolor{gray}{\textbf{64.5}}        & \textcolor{gray}{\textbf{62.8}}                            & 2.0    \\ 
\hline
\end{tabular}
\captionsetup{width=\textwidth} % Center the caption
\caption{Quantitative results of Average Recall(AR) on BOP5 core benchmark datasets for unseen object pose estimation task. Our method exhibits superior performance by large margins compared to other baselines without any refinement. The results are boosted after applying multi-hypothesis and ICP refinements or Megapose-RGB refiner.\ben{All tables could be adjusted to more modern style using toprule midrule bottom...}}
\label{tbl:main table}
\end{table*}




% \begin{table*}[t]
% \centering
% % \begin{tabular}{@{\hspace{5pt}}l@{\hspace{1pt}}c@{\hspace{5pt}}c@{\hspace{1pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}@{\hspace{5pt}}}
% \begin{tabular}{@{\hspace{5pt}}l@{\hspace{5pt}}ccccccccccc}
% \hline
% \multirow{2}{*}{Method}& \multirow{2}{*}{Multi-hypo.} & \multicolumn{2}{c}{Instance Localization}  & \multirow{2}{*}{Refinement} & \multirow{2}{*}{LMO} & \multirow{2}{*}{TLESS} & \multirow{2}{*}{TUDL} & \multirow{2}{*}{ICBIN} & \multirow{2}{*}{YCBV} & \multirow{2}{*}{Mean}\\
% &  &zero-shot &trained & & & & & & &\\ \hline
% ZeroPose & & \ding{51} & & &26.0 & 17.8 & 41.2 & 17.7 & 25.7 & 33.1 \\
% OSOP & & \ding{51} & & &39.3 & - & - & - & \textbf{52.9} &- \\
% Ours(Fast) & & \ding{51} & & &\textbf{52.6} &\textbf{ 42.9} &\textbf{ 70.0} & \textbf{36.7} & 50.5 & \textbf{46.7} \\
% \hdashline
% OSOP & \ding{51} & \ding{51} & & &46.2 & - & - & - & 54.2 & - \\
% Ours(Fast) & \ding{51} & \ding{51} & & &\textbf{56.2} & \textbf{50.6} & \textbf{75.6} & \textbf{42.2} & \textbf{60.8} & \textbf{55.4}\\
% \hline
% DrostPPF & \ding{51} & \ding{51} & &\ding{51} &52.7 & - & - & - & 34.4 & - \\
% PPF + Zephyr & \ding{51} & \ding{51} & &\ding{51} &59.8 & - & - & - & 51.6 & - \\
% OSOP & \ding{51} & \ding{51} & &\ding{51} &48.2 & - & - & - & 57.2 & - \\
% ZeroPose & \ding{51} & \ding{51} & &\ding{51} &49.1  &34.0 & 74.5 & 39.0 & 57.7 & 59.4 \\
% Ours(Fast) & \ding{51} & \ding{51} & &\ding{51} &\textbf{63.5} & \textbf{54.7} & \textbf{89.8} & \textbf{44.2} & \textbf{72.6} & \textbf{64.7} \\
% \hline
% ZeroPose & & & \ding{51} & &26.1 & 24.3 & 61.1 & 24.7 & 29.5 & 33.1 \\
% MegaPose &\ding{51} & & \ding{51} & &18.7 & 19.7 & 20.5 & 15.3 & 13.9 & 17.6 \\
% OVE6D & \ding{51} & & \ding{51} & &62.7 & 52.3 & - & - & - & - \\
% GCPose & \ding{51} & & \ding{51} & &65.2 & 67.9 & 92.6 & - & - & - \\
% Ours(Accurate) & \ding{51} & & \ding{51} & &\textbf{66.8} & 65.1 & \textbf{93.1} & \textbf{43.9} & \textbf{65.8} & \textbf{66.9}\\
% \hline
% OVE6D & \ding{51} & & \ding{51} & \ding{51}&62.7 & 54.6 & - & - & - & - \\
% HybridPPF & \ding{51} & & \ding{51} & \ding{51}&63.1 & 65.5 & 92.0 & - & - & - \\
% Megapose & \ding{51} & & \ding{51} & \ding{51}&58.3 & 54.3 & 71.2 & 37.1 & 63.3 & 56.8 \\
% ZeroPose & \ding{51} & & \ding{51} & \ding{51}&56.2 & 53.3 & 87.2 & 41.8 & 58.4 & 59.4 \\
% Ours(Accurate) & \ding{51} & & \ding{51} & \ding{51} &\textbf{68.0} & \textbf{66.8} & \textbf{95.7} & \textbf{47.4} & \textbf{75.6} & \textbf{70.7} \\ 

% % Ours                    & \ding{51}   & \ding{51}              &                    & \ding{51}                           & \textcolor{gray}{\textbf{61.1}}        & \textcolor{gray}{\textbf{55.7}}        & \textcolor{gray}{\textbf{85.4}}        & \textcolor{gray}{\textbf{47.2}}        & \textcolor{gray}{\textbf{64.5}}        & \textcolor{gray}{\textbf{62.8}}                            & 2.0    \\
% \hline

% \end{tabular}
% \captionsetup{width=\textwidth} % Center the caption
% \caption{Quantitative results of Average Recall(AR) on BOP5 core benchmark datasets for unseen object pose estimation task. Our method exhibits superior performance by large margins compared to other baselines without any refinement. The results are boosted after applying multi-hypothesis and ICP refinements.}
% \label{tbl:main table}
% \end{table*}



% \begin{table*}[t]
% \centering
%     \begin{tabular}{lcccccccccc}
%     \hline
%     \multirow{2}{*}{Method} & \multicolumn{2}{c}{Instance Localization} & \multirow{2}{*}{LMO} & \multirow{2}{*}{TLESS} & \multirow{2}{*}{TUDL} & \multirow{2}{*}{ICBIN} & \multirow{2}{*}{YCBV} & \multirow{2}{*}{HB} & \multirow{2}{*}{ITODD} & \multirow{2}{*}{Mean} \\
%       & zero-shot & trained & & & & & & & &\\ \hline
%     % ZeroPose & & \ding{51} & & 26.0 & 17.8 & 41.2 & 17.7 & 25.7 & 33.1 \\
%     % OSOP & & \ding{51} & & 39.3 & - & - & - & 52.9 & \\
%     % Ours(Fast) & & \ding{51} & & 52.6 & 42.9 & 70.0 & 36.7 & 50.5 & 46.7 \\
%     % \hdashline
%     % OSOP & \ding{51} & \ding{51} & & 46.2 & - & - & - & 54.2 & \\
%     % Ours(Fast) & \ding{51} & \ding{51} & & 56.2 & 50.6 & 75.6 & 42.2 & 52.5 & 55.4 \\
%     % \hline
%     DrostPPF & \ding{51} & & 52.7 & - & - & - & 34.4 & 67.1 & -& - \\
%     PPF + Zephyr  & \ding{51} & & 59.8 & - & - & - & 51.6 & - & -& - \\
%     OSOP & \ding{51} & & 48.2 & - & - & - & 57.2 & 60.5 & -& - \\
%     ZeroPose & \ding{51} & & 49.1 & 34.0 & 74.5 & 39.0 & 57.7 & - & -& 59.4 \\
%     Ours  & \ding{51} & & \textbf{63.5} & \textbf{54.7} & \textbf{89.5} & \textbf{44.2} & \textbf{72.6} & - & - & \textbf{64.9} \\
%     % \hline
%     % ZeroPose & & & \ding{51} & 26.1 & 24.3 & 61.1 & 24.7 & 29.5 & 33.1 \\
%     % MegaPose & & & \ding{51} & 18.7 & 19.7 & 20.5 & 15.3 & 13.9 & 17.6 \\
%     % OVE6D & \ding{51} & & \ding{51} & 62.7 & 52.3 & - & - & - & - \\
%     % GCPose & \ding{51} & & \ding{51} & 65.2 & 67.9 & 92.6 & - & - & - \\
%     % Ours & \ding{51} & & \ding{51} & 66.8 & 68.4 & 93.1 & 46.2 & 65.8 & \\
%     \hline
%     OVE6D  & & \ding{51} & 62.7 & 54.6 & - & - & - & - & -& - \\
%     HybridPPF  & & \ding{51} & 63.1 & 65.5 & 92.0 & - & - & - & -& - \\
%     GCPose & & \ding{51}   & 65.2 & 67.9 & 92.6 & - & - & - & - & - \\
%     Megapose  & & \ding{51} & 58.3 & 54.3 & 71.2 & 37.1 & 63.3 & 75.7 & 40.4 & 56.8 \\
%     ZeroPose  & & \ding{51} & 56.2 & 53.3 & 87.2 & 41.8 & 58.4 & 68.2 & 43.6 & 59.4 \\
%     Ours  & & \ding{51} & \textbf{68.0} & \textbf{66.8} & \textbf{95.7} & \textbf{47.4} & \textbf{75.6} & \textbf{78.2} & \textbf{45.9} & \textbf{70.7} \\
%     \hline
%     \end{tabular}
%     \captionsetup{width=\textwidth}
%     \caption{Quantitative results of Average Recall(AR) on BOP5 core benchmark datasets for unseen object pose estimation task.
%      Our method exhibits superior performance by large margins compared to other baselines without any refinement. The results 
%      are boosted after applying multi-hypothesis and ICP refinement}
% \end{table*}


% To evaluate our generic pose estimation performance, we compared the baselines that are also generalizable to unseen objects. without zero-shot setting and the latest zero-shot pose estimation methods. The zero-shot task can not achieve any object prior which is quite challenging and has performance limitations compared with the supervised method. Since current pose refinement methods can generalize to unseen objects, the biggest challenge is the pose initialization. 
 


\subsection{Ablation study}
\todo Effect of bridged latent matching loss.
\junwen{add another experiment on the coarse loss}

\todo Effect of fine-loss
\junwen{actually without fine-loss it does not work}

\paragraph{The effect of our RGB-D fusion framework.}
\junwen{there is other fusion method like concatenating, which is not applicable in our case. }


\junwen{ \\
Table \ref{tbl:compare to ffb}: compare with other rgbdfusion backbone.}

\begin{table}[t]
\vspace{-0.5cm}
\centering
\begin{tabular}{@{\hspace{5pt}}l@{\hspace{10pt}}c@{\hspace{10pt}}c@{\hspace{10pt}}c@{\hspace{10pt}}c@{\hspace{5pt}}}
\hline
    Method  &Detector &Pose & ADD-0.1d\\ \hline
    DenseFusion  & trained  &trained   & - \\
    FFB6D  & trained  &trained   & 66.2 \\
    Ours(1hypo)   & trained  &trained & \textbf{68.8} \\
    Ours(1hypo)   &zero-shot &zero-shot & 61.7 \\
    Ours(20hypo)   &zero-shot &zero-shot & \textbf{70.8} \\
    Ours(50hypo)   &zero-shot &zero-shot & \textbf{73.1} \\
    % Ours   & \ding{55} & \ding{51}  & 68.4 \\
    % Ours   & \ding{55}  &\ding{51}  &  70.8\\ 
\hline
\end{tabular}
\caption{Quantitative evaluation of 6D pose (ADD-0.1d) on
the Occlusion-LineMOD dataset. Our method achieves comparable results even when conducting unseen object pose estimation and outperforms the baselines in seen object pose estimation fashion \ben{add trained version of ours with 1 hypo}.}
\label{tbl:compare to ffb}
\end{table}


\paragraph{Evaluation of correspondence quality.}
\junwen{\\
Table \ref{tbl:ablation ransac}:ablation of ransac iterations}.

\begin{table}[h]
\vspace{-0.5cm}
\centering
\begin{tabular}{cccc}
\hline
    {Method} & {Sample iter.} & {AR} & {Time} \\ \hline
    Ours & 300k & 62.5 &33.8 \\ 
    Ours & 100k & 59.1 &11.7\\ 
    Ours & 50k  & 58.4 &6.04\\ 
    Ours & 10k  & 55.3 &1.28\\ 
    \textbf{Ours} & 5k   & 52.6 &0.08\\ \hline
\end{tabular}
\caption{Quantitative analysis of 6D pose Average Recall(AR) on
Occlusion-LineMOD dataset for our method with different numbers of sample iterations when applying RANSAC algorithm for our produced correspondences.}
\label{tbl:ablation ransac}
\end{table}

\paragraph{Extracting dense symmetry-agnostic 3D representation.}
\textcolor{red}{visualization of latent embedding.}

% \begin{table}[t]
% % \vspace{-1cm}
% \centering
% \begin{tabular}{lccc}
% \hline
%     Method  & Detection &  Pose estimation & AR\\ \hline
%     GCPose  & Trained  & Zero-shot  & 65.2  \\
%     Ours   & Trained  & Zero-shot  &  \\
%     Ours   & Zero-shot  & Zero-shot  & 61.1 \\ \hline
%     GCPose  & GT  & Zero-shot  & 74.1 \\
%     Ours   & GT  & Zero-shot  &  \\ \hline
% \end{tabular}
% \caption{Quantitative comparison with GCPose on LMO dataset. }
% \label{tbl:compare to gcpose}
% \end{table}

\paragraph{Ablation study for our backbone.}
\junwen{ \\
Table \ref{tbl:compare to roitr}: ablation study with roitr backbone.}
\begin{table}[t]
\vspace{-1cm}
\centering
\begin{tabular}{@{\hspace{5pt}}l@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}}
\hline
    Method    & LMO  & TLESS & ICBIN & TUDL & YCBV \\ \hline
    RoITr w/ RGB & 36.9 & 30.2  & 29.8  & 46.3 & 42.3 \\
    Ours w/o RGB    & 31.6 & 29.3  & 25.9  & 45.8 & 28.6 \\
    Ours w/o BL     \\
    Ours      & \textbf{52.6} & \textbf{42.9}  & \textbf{36.7}  & \textbf{70.0 } & \textbf{50.5} \\ \hline
\end{tabular}
\caption{Quantitative comparison of Average Recall(AR) on BOP-5 datasets.We compare our method with 1)RoITr, where we use the original initialization of the point feature; 2)RoITr+Color, where we initialize the point feature with its RGB value.\ben{add mean AND ablation of RGB or rename "RoITr" to "Ours w/o RGB" and also change order then.}}
\label{tbl:compare to roitr}
\end{table}

\paragraph{Effect of multi-hypothesis.}

\junwen{\\
Table \ref{tbl:ablation hypo}: ablation of multi-hypo}.
\begin{table}[t]
\centering
\vspace{-0.5cm}
\begin{tabular}{cccc}
\hline
        {Method} & {Num. hypo}  & {AR} &{Time}\\ \hline
        Ours & 1   & 52.6 &0.07\\ 
        % Ours & 10  & 54.9 &1.03\\ 
        \textbf{Ours} & 20  & 56.2 &1.03\\ 
        % Ours & 30  & 56.9 &2.79\\ 
        % Ours & 40  & 56.9 &2.79\\ 
        Ours & 50  & 58.2 &3.12\\ 
        Ours & 100  &58.3 &7.26\\ 
        \hline
\end{tabular}
\caption{Quantitative evaluation of Average Recall(AR) on
LMO dataset for our method with different numbers of hypotheses without refinement.}
\label{tbl:ablation hypo}
\end{table}


\paragraph{Effect of refinements.}

\junwen{\\
Table \ref{tbl:ablation refine}: ablation of ICP(depth) and megapose(RGB).}

\begin{table}[t]
\centering
\vspace{-0.5cm}
\begin{tabular}{ccccc}
\hline
{Method} & {RGB Verification} & {ICP} & {AR} & {Time}\\ \hline
Ours &  &  & 56.2 & 0.07 \\
Ours & \ding{51} &  & 61.1 & 0.07 \\ 
Ours &  & \ding{51} & 63.5 & 1.03 \\ 
Ours & \ding{51} & \ding{51} & 65.4 &1.03 \\ 
\hline
\end{tabular}
\caption{Quantitative evaluation of Average Recall(AR) on
LMO dataset for our method when performing different refinement methods.}
\label{tbl:ablation refine}
\end{table}



% \paragraph{Data efficiency.}

% \textcolor{red}{Table \ref{tbl:ablation train obj}: ablation on training objects.}

% \begin{table}[t]
% \centering
% \vspace{-1cm}
% \begin{tabular}{cccc}
% \hline
% {Method} & {Train. obj.}& {Val. obj.} &  {AR} \\ \hline
% Ours & 800  & 200  &  \\ 
% Ours & 400  & 100  &  \\ 
% Ours & 80   & 20   &   \\ \hline
% \end{tabular}
% \caption{Quantitative evaluation of Average Recall(AR) on
% LMO dataset for our method with different number of training objects from GSO.}
% \label{tbl:ablation train obj}
% \end{table}


